Survey on Factuality in Large Language Models: Knowledge, Retrieval and Domain-Specificity

This survey addresses the crucial issue of factuality in Large Language Models (LLMs). As LLMs find applications across diverse domains, the reliability and accuracy of their outputs become vital. We define the Factuality Issue as the probability of LLMs to produce content inconsistent with established facts. We first delve into the implications of these inaccuracies, highlighting the potential consequences and challenges posed by factual errors in LLM outputs. Subsequently, we analyze the mechanisms through which LLMs store and process facts, seeking the primary causes of factual errors. Our discussion then transitions to methodologies for evaluating LLM factuality, emphasizing key metrics, benchmarks, and studies. We further explore strategies for enhancing LLM factuality, including approaches tailored for specific domains. We focus two primary LLM configurations standalone LLMs and Retrieval-Augmented LLMs that utilizes external data, we detail their unique challenges and potential enhancements. Our survey offers a structured guide for researchers aiming to fortify the factual reliability of LLMs.

==> figures/enhance_fig_4sub.tex <==

\begin{figure*}[h]
    \centering
    % \hspace{-.1in}
    \includegraphics[width=4in]{figures/enhancement_4sub.pdf}
    \vspace{-2mm}
    \caption{An overview of methods to enhance factuality in large language models. This encompasses three primary areas: enhancement techniques for pure LLMs and strategies for retrieval-augmented LLMs. %\wjd{This is so small. Why not make a table like previous sections?}
    }
    \vspace{-3mm}
    \label{fig:enhancement}
\end{figure*}
    

==> figures/fig-tree-no-ref.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzset{
leaf/.style={
my-box,
minimum height=1.5em,
fill=hidden-pink!20, % Change the RGB values to the desired values
text=black,
align=left,
font=\footnotesize,
inner xsep=2pt,
inner ysep=4pt,
line width=0.8pt
}
}
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}
        {\begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=6em,font=\normalsize,}{},
            where level=2{text width=9em,font=\normalsize,}{},
            where level=3{text width=9em,font=\normalsize,}{},
            where level=4{text width=7em,font=\normalsize,}{},
            [
                Factuality
                [
                    The Issue\\
                    [
                        Definition 
                    ]
                    [
                        Setting 
                        [
                            Standalone LLMs
                            [
                                ChatGPT~\citep{chatgpt}{, } GPT-4~\citep{GPT4}{, }\\BARD \citep{bard}\\
                                 , leaf, text width=25em
                            ]
                        ]
                        [
                            Retrieval Aug-\\mented LLMs
                            [
                                BingChat \citep{BingChat}{,} Llama-Index \citep{LlamaIndex}{,}
                                , leaf, text width=25em
                            ]
                        ]
                    ]
                    [
                        Impact 
                        [
                            Legal
                            [
                                 \citet{curran2023hallucination}{,} \citet{Pranshu2023}{,} \citet{news_mayor}
                                , leaf, text width=25em
                            ]
                        ]
                        [
                            Medicine
                            [
                                \citet{nori2023capabilities}{,} \citet{shen2023chatgpt}{,} \citet{USMLE_evaluation}
                                , leaf, text width=25em
                            ]
                        ]
                    ]
                    
                ]
                
                [
                    Evaluation\\
                    [
                        Factuality Evaluation\\Benchmark 
                        [
                            MMLU~\citep{MMLU}{, } TruthfulQA~\citep{TruthfulQA}{, }\\C-Eval~\citep{C-Eval}{, } AGIEval~\citep{AGIEval}{, } \\ RealTimeQA~\citep{kasai2022realtimeqa}{, } FreshQA~\citep{vu2023freshllms}, leaf, text width=33em
                        ]
                    ]
                    [
                        Factuality\\Evaluation 
                        [
                            SelfCheckGPT~\citep{SelfCheckGPT}{, } FActScore~\citep{Min2023-FActScore}{, } \\ \citet{wang2023evaluating}{, } \citet{yu2023generate}{, } \citet{kadavath2022language}, leaf, text width=33em
                        ]
                    ]
                    % [
                    %     Evaluating\\Factuality\\Evaluation
                    %     [
                    %         , leaf, text width=33em
                    %     ]
                    % ]
                    [
                        Domain-Factuality\\Evaluation 
                        [ 
                            FLARE (Finance) \citep{xie2023pixiu}{, } CMB (Medicine) \citep{wang2023cmb}{, }\\GeneTuring (Gene) \citep{jin2023genegpt}{, } EcomInstruct (Ecom) \citep{li2023ecomgpt}, leaf, text width=33em
                        ]
                    ]
                ]
                [
                    Analysis
                    [
                        Factuality Analysis
                        [
                            Knowledge Storage \\
                            Knowledge Completeness and Awareness \\
                            Contextual Influence and Knowledge Conflict , leaf, text width=27em 
                        ]
                    ]
                    [
                        Error Causes\\
                        [
                            Model-Level 
                            [
                                Domain Knowledge Deficit{, } Outdated Information{, }\\ Immemorization{, } Forgetting{, } Reasoning Failure, leaf, text width=24em
                            ]
                            % [
                            %     Domain Knowledge Deficit, leaf, text width=13em
                            % ]
                            % [
                            %     Outdated Information, leaf, text width=10em
                            % ]
                            % [
                            %     Immemorization, leaf, text width=8em
                            % ]
                            % [
                            %     Forgetting, leaf, text width=5em
                            % ]
                            % [
                            %     Reasoning Failure, leaf, text width=9em
                            % ]
                            
                        ]
                        [
                            Retrieval-Level 
                            [
                                Insufficient Information{, } Distracting Information{, } \\ Misinformation Not Recognized by LLMs{, }\\
                                Misinterpretation of Related Information, leaf, text width=24em
                            ]
                            % [
                            %     Insufficient Information, leaf, text width=13em
                            % ]
                            % [
                            %     Misinformation Not Recognized by LLMs, leaf, text width=18em
                            % ]
                            % [
                            %     Distracting Information, leaf, text width=12em
                            % ]
                            % [
                            %     Misinterpretation of Related Information, leaf, text width=18em
                            % ]
                        ]
                        [
                            Inference-Level 
                            [
                                Snowballing{, } Erroneous Decoding{, } Exposure Bias, leaf, text width=24em
                            ]
                            % [
                            %     Snowballing, leaf, text width=8em
                            % ]
                            % [
                            %     Erroneous Decoding, leaf, text width=12em
                            % ]
                            % [
                            %     Exposure Bias, leaf, text width=12em
                            % ]
                        ]
                    ]
                ]
                % [
                %     Analysis\\
                % ]
                [
                    Enhancement
                    [
                        On Standalone \\LLMs
                        [
                            Pretrain-based
                            [
                                Initial Pretraining: \citet{sadeq-etal-2023-unsupervised}{; }\\
                                Continual Pretraining: TOPICPREFIX \citep{lee2022factuality}\\
                                , leaf, text width=24em
                            ]
                            
                        ]
                        [
                            SFT-based 
                            [
                                Continual SFT: \citet{moiseev-etal-2022-skill}{;}\\
                                Model Editing: \citet{dong-etal-2022-calibrating}{, }\\ CaliNET \citep{huang2023transformerpatcher}{, }  KN \citep{dai-etal-2022-knowledge}{, }\\ T-Patcher \citep{dai-etal-2022-knowledge}{, }
                                SERAC \citep{Mitchell2022MemoryBasedME}\\
                                , leaf, text width=22em
                            ]
                        ]
                        [
                            Multi-Agent 
                            [
                                Multi-debate: \citet{multiagent_debate}\\
                                Multi-role: \citet{cohen2023lm}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Decoding 
                            [
                                \citet{yu2023generate}{,} \citet{chuang2023dola}\\
                                , leaf, text width=18em
                            ]
                        ]
                    ]
                    [
                        On Retrieval-\\Augmented\\LLMs
                        [
                            Normal RAG
                            [
                                \citet{borgeaud2022improving}{, } \citet{LlamaIndex} \\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Interactive\\Retrieval 
                            [
                                CoT-based path: \citet{he2022rethinking}{, } IRCoT \citep{trivedi-etal-2023-interleaving} \\
                                Agent-based Retrieval: ReAct \citep{yao2023react}
                                , leaf, text width=24em
                            ]
                        ]
                        [
                            Retrieval\\Adaptation  
                            [
                                Prompt-based: LLM-Augmenter \citep{peng2023check}{, } \\
                                SFT-based: ATLAS \citep{Atlas}{, } \\REPLUG \citep{REPLUG}{, } SAIL \citep{luo2023sail}  \\
                                RLHF-based: GopherCite \citep{GopherCite}\\
                                , leaf, text width=24em
                            ]
                        ]
                        [
                            Retrieval on External \\ Memory 
                            [
                                 General Knowledge: \citet{li2022decoupled}{,}\\ \citet{houlsby2019parameterefficient}{,} G-MAP \citep{wan2022gmap}  \\
                                Entity Knowledge: knowledge plugin \citep{zhang-etal-2023-plug}\\KALA \citep{KALA} TOME \citep{jong2022mention}{, }  \\
                                , leaf, text width=24em
                            ]
                        ]
                        [
                            Retrieval on\\Structured Data
                            [
                                StructGPT \citep{StructGPT} {, } \citet{zhang2023mitigating}
                                , leaf, text width=24em
                            ]
                        ]
                    ]
                    [
                        Domain Factuality\\Enhanced LLMs
                        \\
                        [
                            Medicine: HuatuoGPT \citep{zhang2023huatuogpt}{, } DISC-MedLLM \citep{ross2022large}\\
                            Legal: LawGPT \citep{nguyen2023brief}{, } ChatLaw \citep{cui2023chatlaw}\\
                            Finance: EcomGPT \citep{li2023ecomgpt}{, } BloombergGPT \citep{BloombergGPT} \\
                            Education: GrammarGPT \citep{fan2023grammargpt}\\
                                , leaf, text width=30em
                        ]
                    ]
                    
                ]
                % [
                %     Data 
                %     [
                %         Instructions From \\ Human  (\S )
                %         [
                %             NLP Benchmarks
                %             [                            
                %                 PromptSource~\citep{bach-etal-2022-promptsource}{, }SuperNaturalInstruction~\citep{wang-etal-2022-super}{, } \\ FLAN~\citep{longpre2023flan}{, }Unnatural Instructions~\citep{DBLP:journals/corr/abs-2212-09689}{, } \\
                %                 OIG~\citep{OIG}
                %                 , leaf, text width=33em
                %             ]
                %         ]
                %         [
                %             Hand-crafted Instructions
                %             [
                %                 Dolly-v2~\citep{DatabricksBlog2023DollyV2}{, } OpenAssistant~\citep{Kopf2023OpenAssistantC}{, } \\
                %                 COIG~\citep{Zhang2023ChineseOI}{,} ShareGPT~\citep{vicuna2023}{,} 
                %                 , leaf, text width=33em
                %             ]
                %         ]
                %     ]
                %     [
                %         Instruction From \\ Strong LLMs (\S )
                %         [
                %             Self-Instruct
                %             [
                %                 Improving \\ Input Quality
                %                 [
                %                     Self-Instruction~\citep{DBLP:journals/corr/abs-2212-10560}{, } Lamini-lm~\citep{DBLP:journals/corr/abs-2304-1440}{, } \\ Baize~\citep{DBLP:journals/corr/abs-2304-01196}{, } AttrPrompt~\citep{yu2023large}{, }\\ WizardLM~\citep{xu2023wizardlm}{, } WizardCoder~\citep{luo2023wizardcoder}{, }\\
                %                     Unnatural Instructions~\citep{DBLP:journals/corr/abs-2212-09689}{, } Phi-1~\citep{gunasekar2023textbooks}
                %                     , leaf, text width=33em
                %                 ]
                %             ]
                %             [
                %                 Improving \\Output Quality
                %                 [
                %                     CoT~\citep{wei2022chain}{, }Orca~\citep{mukherjee2023orca}{, }Lion~\citep{Jiang2023LionAD}\\
                %                     Self-Alignment~\citep{Sun2023PrincipleDrivenSO}{, }Phoenix~\citep{DBLP:journals/corr/abs-2304-10453}{, }\\
                %                     Expert Prompting~\citep{xu2023expertprompting}
                %                     , leaf, text width=33em
                %                 ]
                %             ]
                %         ]
                %         [
                %             Multi-Turn Instructions
                %             [
                %                 Baize~\citep{DBLP:journals/corr/abs-2304-01196}{, }CAMEL~\citep{DBLP:journals/corr/abs-2303-17760}{, }SelFee~\citep{selfee2023}{, }\\UltraLLaMA~\citep{ding2023enhancing}{, } Vicuna~\citep{vicuna2023} 
                %             , leaf, text width=33em
                %             ]
                %         ]
                %         [
                %             Multilingual Instructions
                %             [
                %                 Phoenix~\citep{DBLP:journals/corr/abs-2304-10453}{, }BayLing~\citep{Zhang2023BayLingBC}{, }\\ BactrianX~\citep{bactrian}
                %             , leaf, text width=33em
                %             ]
                %         ]
                %     ]
                % ]
                % [
                %     111
                %     [
                %         Instruction Data \\ Management (\S )
                %         [
                %             Instruction Implications
                %             [
                %                 \textsc{T\"ulu}~\citep{wang2023far}{, } FLACUNA~\citep{ghosal2023flacuna}{, } \\
                %                 Data-Constrained LM~\citep{muennighoff2023scaling}{, }  BELLE~\citep{DBLP:journals/corr/abs-2304-07854}
                %                 , leaf, text width=33em
                %             ]
                %         ]
                %         [
                %             Instruction Quantity
                %             [
                %                 IFS~\citep{alshikh2023becoming}{, }LIMA~\citep{zhou2023lima}{, } \\
                %                 Instruction Mining~\citep{cao2023instruction}{, }
                %                 Alpagasus~\citep{chen2023alpagasus}
                %                 , leaf, text width=33em
                %             ]
                %         ]
                %     ]
                % ]
            ]
        \end{forest}}
        \vspace{-4mm}
    \caption{Taxonomy of research in factuality in Large Language Models (LLMs) that consists of the issue, causes, evaluation, analysis, and enhancement methods.}
    \label{fig:tree}
\end{figure*}

==> figures/fig-tree_4sub.tex <==
\definecolor{mycolor}{RGB}{215, 245, 200}

\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzset{
leaf/.style={
my-box,
minimum height=1.5em,
fill=mycolor, % Change the RGB values to the desired values
text=black,
align=left,
font=\footnotesize,
inner xsep=2pt,
inner ysep=4pt,
line width=0.8pt
}
}
\begin{figure*}[t!]
    \centering
    \begin{adjustbox}{width=0.9\textwidth}
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=6em,font=\normalsize,}{},
            where level=2{text width=9em,font=\normalsize,}{},
            where level=3{text width=9em,font=\normalsize,}{},
            where level=4{text width=7em,font=\normalsize,}{},
            [
                Factuality
                [
                    The Issue\\(Sec \ref{sec:the_issue})
                    [
                        Definition (Sec \ref{sec:definition})
                    ]
                    [
                        Setting (Sec \ref{sec:definition})
                        [
                            Standalone LLMs
                            [
                                ChatGPT~\citep{chatgpt}{, } GPT-4~\citep{GPT4}{, }\\BARD \citep{bard}\\
                                 , leaf, text width=15em
                            ]
                        ]
                        [
                            Retrieval Aug-\\mented LLMs
                            [
                                BingChat \citep{BingChat}{,} Llama-Index \citep{LlamaIndex}
                                , leaf, text width=15em
                            ]
                        ]
                    ]
                ]
                [
                    Evaluation\\(Sec \ref{sec:evalution})
                    [
                        Factuality Evaluation\\Benchmark \ref{sec:eval_benchmark}
                        [
                            MMLU~\citep{MMLU}{, } TruthfulQA~\citep{TruthfulQA}{, }\\C-Eval~\citep{C-Eval}{, } AGIEval~\citep{AGIEval}{, } \\ RealTimeQA~\citep{kasai2022realtimeqa}{, } FreshQA~\citep{vu2023freshllms}, leaf, text width=24em
                        ]
                    ]
                    [
                        Factuality\\Evaluation \ref{sec:factuality-eval}
                        [
                            SelfCheckGPT~\citep{SelfCheckGPT}{, } FActScore~\citep{Min2023-FActScore}{, } \\ \citet{wang2023evaluating}{, } \citet{yu2023generate}{, } \citet{kadavath2022language}, leaf, text width=24em
                        ]
                    ]
                ]
                [
                    Analysis\\
                    (Sec \ref{sec:analysis})
                    [
                        Factuality Analysis\\
                        (Sec \ref{sec:factuality_analysis})
                        [
                            Knowledge Storage (Sec \ref{sec:analy_store})\\
                            Knowledge Completeness and Awareness (Sec \ref{sec:analy_aware})\\
                            Contextual Influence and Knowledge Conflict (Sec \ref{sec:analy_confict}), leaf, text width=27em 
                        ]
                    ]
                    [
                        Error Causes\\(Sec \ref{sec:causes})
                        [
                            Model-Level \ref{sec:model-causes}
                            [
                                Domain Knowledge Deficit{, } Outdated Information{, }\\ Immemorization{, } Forgetting{, } Reasoning Failure, leaf, text width=18em
                            ]
                        ]
                        [
                            Retrieval-Level \ref{sec:retrieval-causes}
                            [
                                Insufficient Information{, } Distracting Information{, } \\ Misinformation Not Recognized by LLMs{, }\\
                                Misinterpretation of Related Information, leaf, text width=18em
                            ]
                        ]
                        [
                            Inference-Level \ref{sec:inference-causes}
                            [
                                Snowballing{, } Erroneous Decoding{, } Exposure Bias, leaf, text width=18em
                            ]
                        ]
                    ]
                ]
                [
                    Enhancement\\ (Sec \ref{sec:enhancement})
                    [
                        On Standalone\\LLMs
                        (Sec \ref{sec:enhace_pure})
                        [
                            Pretrain-based
                            \ref{sec:enhace_pure}
                            [
                                Initial Pretraining: \citet{sadeq-etal-2023-unsupervised}{; }\\
                                Continual Pretraining: TOPICPREFIX \citep{lee2022factuality}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            SFT-based \ref{sec:enhace_pure_sft}
                            [
                                Continual SFT: \citet{moiseev-etal-2022-skill}{;}\\
                                Model Editing: \citet{dong-etal-2022-calibrating}{, }\\ CaliNET \citep{huang2023transformerpatcher}{, }  KN \citep{dai-etal-2022-knowledge}{, }\\ T-Patcher \citep{dai-etal-2022-knowledge}{, }
                                SERAC \citep{Mitchell2022MemoryBasedME}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Multi-Agent \ref{sec:enhace_pure_multi}
                            [
                                Multi-debate: \citet{multiagent_debate}\\
                                Multi-role: \citet{cohen2023lm}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Decoding \ref{sec:enhace_pure_decoding}
                            [
                                \citet{lee2022factuality}{,} \citet{chuang2023dola}\\
                                , leaf, text width=18em
                            ]
                        ]
                    ]
                    [
                        On Retrieval-\\Augmented\\LLMs(Sec \ref{sec:enhace_rag})
                        [
                            Normal RAG
                            \ref{sec:enhace_rag_normal})
                            [
                                \citet{borgeaud2022improving}{, } \citet{LlamaIndex} \\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Interactive\\Retrieval \ref{sec:enhace_rag_inter}
                            [
                                CoT-based path: \citet{he2022rethinking}{, } IRCoT \citep{trivedi-etal-2023-interleaving} \\
                                Agent-based Retrieval: ReAct \citep{yao2023react}
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval\\Adaptation  \ref{sec:enhace_rag_adapt}
                            [
                                Prompt-based: LLM-Augmenter \citep{peng2023check}{, } \\
                                SFT-based: ATLAS \citep{Atlas}{, } \\REPLUG \citep{REPLUG}{, } SAIL \citep{luo2023sail}  \\
                                RLHF-based: GopherCite \citep{GopherCite}\\
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval on External \\ Memory \ref{sec:enhace_rag_mem}
                            [
                                 General Knowledge: \citet{li2022decoupled}{,}\\ \citet{houlsby2019parameterefficient}{,} G-MAP \citep{wan2022gmap}  \\
                                Entity Knowledge: knowledge plugin \citep{zhang-etal-2023-plug}\\KALA \citep{KALA} TOME \citep{jong2022mention}{, }  \\
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval on\\Structured Data
                            \ref{sec:enhace_rag_kg}
                            [
                                StructGPT \citep{StructGPT} {, } \citet{zhang2023mitigating}
                                , leaf, text width=16em
                            ]
                        ]
                    ]
                ]
            ]
        \end{forest}
    \end{adjustbox}
        \vspace{-4mm}
    \caption{Taxonomy of research on factuality in Large Language Models that consists of the issue, evaluation, analysis and enhancement.}
    \label{fig:tree}
\end{figure*}

==> sections/Causes.tex <==

Understanding the root causes of these factual inaccuracies is crucial for refining these models and ensuring their reliable application in real-world scenarios. In this subsection, we delve into the multifaceted origins of these errors, categorizing them based on the stages of model operation: Model Level, Retrieval Level, Generation Level, and other miscellaneous causes. Table~\ref{tab:causes} shows examples of factuality errors caused by different factors.


\subsubsection{Model-level Causes}
\label{sec:model-causes}
This subsection delves into the intrinsic factors within large language models that contribute to factual errors, originating from their inherent knowledge and capabilities. 

\paragraph{Domain Knowledge Deficit} The model may lack comprehensive expertise in specific domains, leading to inaccuracies. Every LLM has its limitations based on the data it was trained on. If an LLM hasn't been exposed to comprehensive data in a specific domain during its training, it's likely to produce inaccurate or generalized outputs when queried about that domain. For instance, while an LLM might be adept at answering general science questions, it might falter when asked about niche scientific subfields \citep{ScienceQA}.

\paragraph{Outdated Information} The model's dependence on older datasets can make it unaware of recent developments or changes. LLMs are trained on datasets that, at some point, become outdated. This means that any events, discoveries, or changes post-dating the last training update won't be known to the model. For example, ChatGPT and GPT-4 are both trained on data up to 2021.09 might not be aware of events or advancements after then.

\paragraph{Immemorization} The model does not always retain knowledge from its training corpus. While it's a misconception that LLMs ``memorize" data, they do form representations of knowledge based on their training. However, they might not always recall specific, less-emphasized details from their training parameters, especially if such details were rare or not reinforced through multiple examples. For example, ChatGPT has pretrained with Wikipedia, but it still fail in answering some questions from NaturalQuestions \citep{NQ} and TriviaQA \citep{TQ}, which are constructed from Wikipedia \citep{wang2023evaluating}.

\paragraph{Forgetting} The model might not retain knowledge from its training phase or could forget prior knowledge as it undergoes further training. As models are further fine-tuned or trained on new data, there's a risk of ``catastrophic forgetting" ~\citep{goodfellow2015empirical, wang2022preserving, chen2020recall, zhai2023investigating} where they might lose certain knowledge they were previously know. This is a well-known challenge in neural network training, where networks forget previously learned information when exposed to new data, which also happens in large language models \citep{luo2023empirical}.

\paragraph{Reasoning Failure} While the model might possess relevant knowledge, it can sometimes fail to reason with it effectively to answer queries. Even if an LLM has the requisite knowledge to answer a question, it might fail to connect the dots or reason logically. For instance, ambiguity in the input~\citep{liu2023we} can potentially lead to a failure in understanding by LLMs, consequently resulting in reasoning errors. In addition, \citet{berglund2023reversal} find the LLM traps in the reversal curse, for example, it knows that A is B's mother but fail to answer who is B's son. This is especially evident in complex multi-step reasoning tasks or when the model needs to infer based on a combination of facts \citep{tan2023chatgpt,kotha2023understanding}. 

% For instance, while it 

% Multi-modal Deficit: Challenges emerge when the model must process multiple types of data, such as text and images, and struggles to integrate them cohesively. Most LLMs are designed to process textual information. When faced with tasks that require understanding or generating content across multiple modalities (like visual and textual), they might struggle \citep{}. For instance, spatial reasoning or interpreting visual cues alongside text can be challenging for models that aren't specifically trained on multi-modal data.


\subsubsection{Retrieval-level Causes}
\label{sec:retrieval-causes}
The retrieval process plays a pivotal role in determining the accuracy of LLMs' responses, especially in retrieval-augmented settings. Several factors at this level can lead to factual errors:

\paragraph{Insufficient Information}
If the retrieved data doesn't provide enough context or details, the LLM might struggle to generate a factual response. This can result in generic or even incorrect outputs due to the lack of comprehensive evidence.

\paragraph{Misinformation Not Recognized by LLMs}
LLMs can sometimes accept and propagate misinformation present in the retrieved data. This is especially concerning when the model encounters knowledge conflicts, where the retrieved information contradicts its pre-trained knowledge, or multiple retrieved documents contradict each other~\cite{TruthDiscovery}. For instance, \cite{longpre2021entity} observed that the more irrelevant the evidence, the more likely the model is to rely on its intrinsic knowledge. Recent studies, such as \cite{pan2023risk}, have also shown that LLMs are susceptible to misinformation attacks within the retrieval process.

\paragraph{Distracting Information}
LLMs can be misled by irrelevant or distracting information in the retrieved data. For example, if the evidence mentions a "Russian movie" and "Directors", the LLM might incorrectly infer that "The director is Russian". \cite{luo2023sail} highlighted this vulnerability, noting that LLMs can be significantly impacted by distracting retrieval results. They further proposed instruction tuning as a potential solution to enhance the model's ability to sift through and leverage retrieval results more effectively.


Additionally, when dealing with long retrieval inputs, the models tend to show their best performance when processing information given at the beginning or end of the input context, according to \citet{liu2023lost}. In contrast, the models are likely to experience a significant decrease in performance when they are required to extract relevant data from the middle of these extensive contexts.
% find that performance tends to be at its peak when relevant information is located at the beginning or end of the input context. Conversely, it experiences a notable decline when models are required to retrieve pertinent information from the middle of lengthy contexts. 

\paragraph{Misinterpretation of Related Information}
Even when the retrieved information is closely related to the query, LLMs can sometimes misunderstand or misinterpret it. While this might be less frequent when the retrieval process is optimized, it remains a potential source of error. For instance, in the ReAct study \citep{yao2023react}, the rate of errors dropped significantly when the retrieval process was improved.

\subsubsection{Inference-level Causes}
\label{sec:inference-causes}
\paragraph{Snowballing} During the generation process, a minor error or deviation at the beginning can compound as the model continues to generate content. %This phenomenon, akin to a snowball growing in size as it rolls downhill, can result in outputs that are not only factually incorrect but also contextually incoherent. 
For instance, if an LLM misinterprets a prompt or starts with an inaccurate premise, the subsequent content can veer further from the truth \citep{Snowball,varshney2023stitch}.

\paragraph{Erroneous Decoding} The decoding phase is crucial for translating the model's internal representations into human-readable content~\citep{chuang2023dola, massarelli2020decoding}. Mistakes during this phase, whether due to issues like beam search errors or suboptimal sampling strategies, can lead to outputs that misrepresent the model's actual "knowledge" or intention. This can manifest as inaccuracies, contradictions, or even nonsensical statements.

\paragraph{Exposure Bias}
LLMs are a product of their training data. If they've been exposed more frequently to certain types of content or phrasing, they might have a bias toward generating similar content, even when it's not the most factual or relevant. This bias can be especially pronounced if the training data has imbalances or if certain factual scenarios are underrepresented~\citep{felkner2023winoqueer, gallegos2023bias}. The model's outputs, in such cases, reflect its training exposure rather than objective factuality. For example, research by ~\cite{hossain-etal-2023-misgendered} suggests that LLMs can correctly identify the gender of individuals who conform to the binary gender system, but they perform poorly when determining non-binary or neutral genders.

==> sections/Domain-Eval.tex <==

\label{sec:domain-eval}
\input{tables/tb-domain-eval}

To assess the performance and factuality of these specialized LLMs, a plethora of datasets and benchmarks have been proposed across various domains. These resources not only serve as critical tools for evaluating the capabilities of LLMs but also facilitate advancements in specialized applications. We summarize them in Table~\ref{tab:domain-eval}. The distinction between this subsection and the previous two lies in its focus. This subsection delves deeper into factuality evaluation tailored to specific domains, while Sec \ref{sec:eval_benchmark} and \ref{sec:factuality-eval} primarily concentrate on general factuality evaluation, with only a portion of their content dedicated to datasets evaluating factuality within specific domains.


{\paragraph{Finance}}
\citet{xie2023pixiu} designed a financial natural language understanding and prediction evaluation benchmark dubbed FLARE, based on their collected financial instruction tuning dataset FIT. This benchmark is used to evaluate their FinMA model. It randomly selects validation sets from FIT to choose the best model checkpoint and utilizes distinct test sets for evaluation.
FLARE is a broader variant compared to the existing FLUE benchmark~\cite{shah2022flue} as it also encapsulates financial prediction tasks like stock movement prediction in addition to standard NLP tasks. 
The FLARE dataset includes several subtasks, such as sentiment analysis (FPB, FiQA-SA), news headline  classification (Headline), named entity recognition (NER), question answering (FinQA, ConvFinQA), and stock movement prediction (BigData22, ACL18, CIKM18).
Performance is gauged via a variety of metrics for each task, such as the accuracy and weighted F1 Score for sentiment analysis, entity-level F1 score for named entity recognition, and accuracy and Matthews correlation coefficient for stock movement prediction.
Several methods, including their own FIT-fine-tuned FinMA and other LLMs (BloombergGPT, GPT-4, ChatGPT, BLOOM, GPT-NeoX, OPT-66B, Vicuna-13B) are dedicated to their comparison. BloombergGPT's performance is assessed in various shot scenarios, while the zero-shot performance is reported for the remaining results. Some of the baselines depend on human evaluations given that LLMs without fine-tuning fail to generate instruction-defined answers. Conversely, FinMA's results are conducted on a zero-shot basis and can be evaluated automatically. 
To enable direct comparison between the performance of FinMA and BloombergGPT, despite the former not releasing their test datasets, test datasets were constructed with the same data distribution.

\citet{li2023ecomgpt} propose EcomInstruct benchmark, which experiment investigates the performance of their EcomGPT language model in comparison to baseline models such as BLOOM and BLOOMZ. Categories of these baseline models include pre-trained large models with decoder-only architecture like BLOOM, and instruction-following language models like BLOOMZ and ChatGPT. The evaluation metric of the EcomInstruct involves converting all tasks to generative paradigms and using text generation evaluation metrics like ROUGE-L. Classification tasks were evaluated with precision, recall, and F1 scores. The EcomInstruct dataset, comprising 12 tasks across four major categories, is divided into training and testing sections. The EcomGPT is trained on 85,746 instances of E-commerce data. The performance of the model is assessed based on its capacity to generalize unseen tasks or datasets, with emphasis on cross-language and cross-task paradigm settings.


{\paragraph{Medicine}}
\citet{wang2023cmb} propose a localized medical benchmark called CMB, or the Comprehensive Medical Benchmark in Chinese. CMB is rooted entirely in the native Chinese linguistic and cultural framework. While traditional Chinese medicine is a significant part of this evaluation, it does not make up the entire benchmark.
Both prominent LLMs, such as ChatGPT and GPT-4, and localized Chinese LLMs, including those specializing in the health domain, are evaluated using CMB. However, the benchmark is not designed as a leaderboard competition, but rather as a tool for self-assessment and understanding the progression of models in this field.
CMB embodies a comprehensive, multi-layered medical benchmark in Chinese, comprised of hundreds of thousands of multiple-choice questions and complex case consultation questions. This wide range of queries covers all clinical medical specialties and various professional levels, seeking to evaluate a model's medical knowledge and clinical consultation capabilities comprehensively.
 
\citet{li2023huatuo} introduce Huatuo-26M dataset, the largest Chinese medical Question and Answer (QA) dataset to date, including over 26 million high-quality medical QA pairs. It covers a wide range of topics, such as diseases, symptoms, treatments, and drug information. The dataset is a valuable resource for anyone looking to improve AI applications in the medical field, such as chatbots and intelligent diagnostic systems.
The Huatuo-26M dataset is gathered and integrated from various sources, including online medical encyclopedias, online medical knowledge bases, and online medical consultation records. Each QA pair in the dataset contains a problem description and a corresponding answer from a doctor or expert. Although a significant proportion of the Huatuo-26M dataset is constituted by the online medical consultation records, the text format data from these records is not publicly available, for unspecified reasons.
This dataset is expected to be instrumental for multiple types of research and AI applications in the medical field. These areas of application extend to Natural Language Processing tasks like developing QA systems, text classification, sentiment analysis, and Machine Learning model training tasks like disease prediction and personalized treatment recommendation. Consequently, the dataset is favorable for developing AI applications in the medical field, from intelligent diagnosis systems to medical consultation chatbots.

% {\paragraph{Gene: }}
\citet{jin2023genegpt} use nine tasks related to NCBI resources to evaluate the proposed GeneGPT model. The dataset used is GeneTuring benchmark~\cite{Hou2023GeneTuring}, which contains 12 tasks with 50 question-answer pairs each. The tasks are divided into four modules - Nomenclature  (Gene alias, Gene name conversion),  Genomic location(Gene SNP association, Gene location, SNP location), 
  Functional analysis(Gene disease association, Protein-coding genes), 
  Sequence alignment (DNA to human genome, DNA to multiple species). Two settings of GeneGPT are assessed: a full setting where all prompt components are used, and a slim setting using only two components. The performance of GeneGPT is compared against various baselines including general-domain GPT-based LLMs like GPT-2, GPT-3, and ChatGPT. Additionally, GPT-2-sized biomedical domain-specific LLMs such as BioGPT and BioMedLM are evaluated. The new Bing, a retrieval-augmented LLM with access to relevant web pages, is also assessed. The result evaluation of the compared methods is based on the results reported in the original benchmark and are manually evaluated. However, the evaluation of the proposed GeneGPT method is determined through automatic evaluations.





\paragraph{Law}
LegalBench~\citep{guha2023legalbench} is a benchmark for legal reasoning introduced due to the increasing use of LLMs in the legal field. It consists of 162 tasks covering six types of legal reasoning and was collaboratively constructed through an interdisciplinary process with significant contributions from legal professionals. The tasks designed aim to either demonstrate practical legal reasoning capabilities or measure reasoning skills that are of interest to lawyers. To facilitate discussions between different fields relating to LLMs in law, LegalBench tasks correspond to popular legal frameworks for describing legal reasoning, thus creating a shared language between lawyers and LLM developers. The paper not only describes LegalBench, but also presents an evaluation of 20 different open-source and commercial LLMs and highlights the types of research opportunities that LegalBench can provide.

LawBench~\citep{fei2023lawbench} is an evaluation framework dedicated to assessing the capabilities of LLMs in relation to legal tasks. The context-specificity and high-stakes nature of the law field make it crucial to have a clear grasp of LLMs' legal knowledge and their ability to execute legal tasks. 
LawBench dives deep into three cognitive evaluations of LLMs: the capability to memorize crucial legal details, understanding legal texts, and applying legal knowledge to resolve complicated legal problems. A total of 20 diverse tasks have been put together, covering five main task categories: single-label classification, multi-label classification, regression, extraction, and generation. 
Throughout the evaluation process, 51 LLMs were extensively tested under LawBench, compiling a spectrum of language models including 20 multilingual LLMs, 22 Chinese-oriented LLMs, and 9 law-specific LLMs. The results concluded that GPT-4 ranked as the superior LLM in the law domain, significantly surpassing its competitors. Despite the noted improvements when LLMs were fine-tuned on law-specific texts, the study acknowledged that there is still a long road ahead in achieving highly reliable LLMs for legal tasks.

\citet{bi2023oceangpt}  design OceanBench to evaluate the capabilities of LLMs for oceanography tasks.
OceanBench includes a total of 15 type of ocean-related tasks, such as question-answering and description tasks.
The samples in OceanBench are are automatically generated from the seed dataset and have undergone manual verification by experts.

==> tables/fig-tree_4sub.tex <==
\definecolor{mycolor}{RGB}{215, 245, 200}

\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzset{
leaf/.style={
my-box,
minimum height=1.5em,
fill=mycolor, % Change the RGB values to the desired values
text=black,
align=left,
font=\footnotesize,
inner xsep=2pt,
inner ysep=4pt,
line width=0.8pt
}
}
\begin{figure*}[t!]
    \centering
    \begin{adjustbox}{width=0.9\textwidth}
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=6em,font=\normalsize,}{},
            where level=2{text width=9em,font=\normalsize,}{},
            where level=3{text width=9em,font=\normalsize,}{},
            where level=4{text width=7em,font=\normalsize,}{},
            [
                Factuality
                [
                    The Issue\\(Sec \ref{sec:the_issue})
                    [
                        Definition (Sec \ref{sec:definition})
                    ]
                    [
                        Setting (Sec \ref{sec:definition})
                        [
                            Standalone LLMs
                            [
                                ChatGPT~\citep{chatgpt}{, } GPT-4~\citep{GPT4}{, }\\BARD \citep{bard}\\
                                 , leaf, text width=15em
                            ]
                        ]
                        [
                            Retrieval Aug-\\mented LLMs
                            [
                                BingChat \citep{BingChat}{,} Llama-Index \citep{LlamaIndex}
                                , leaf, text width=15em
                            ]
                        ]
                    ]
                    [
                        Impact (Sec \ref{sec:impact})
                        [
                            Legal: \citet{curran2023hallucination}{, } \citet{Pranshu2023}{, } \citet{news_mayor}
                                , leaf, text width=24em
                        ]
                        [
                            Medicine: \citet{nori2023capabilities}{,} \citet{shen2023chatgpt}{,} \citet{USMLE_evaluation}
                                , leaf, text width=24em
                        ]
                    ]
                ]
                [
                    Evaluation\\(Sec \ref{sec:evalution})
                    [
                        Factuality Evaluation\\Metrics \ref{sec:eval_metrics}
                        [
                            Rule-based evaluation metrics;
                            Neural evaluation metrics; \\
                            Human evaluation metrics; LLM-based  evaluation metrics, leaf, text width=24em
                        ]
                    ]
                    [
                        Factuality Evaluation\\Benchmark \ref{sec:eval_benchmark}
                        [
                            MMLU~\citep{MMLU}{, } TruthfulQA~\citep{TruthfulQA}{, }\\C-Eval~\citep{C-Eval}{, } AGIEval~\citep{AGIEval}{, } \\ RealTimeQA~\citep{kasai2022realtimeqa}{, } FreshQA~\citep{vu2023freshllms}, leaf, text width=24em
                        ]
                    ]
                    [
                        Factuality\\Evaluation \ref{sec:factuality-eval}
                        [
                            SelfCheckGPT~\citep{SelfCheckGPT}{, } FActScore~\citep{Min2023-FActScore}{, } \\ \citet{wang2023evaluating}{, } \citet{yu2023generate}{, } \citet{kadavath2022language}, leaf, text width=24em
                        ]
                    ]
                    [
                        Domain-Factuality\\Evaluation (Sec \ref{sec:domain-eval})
                        [ 
                            FLARE (Finance) \citep{xie2023pixiu}{, } CMB (Medicine) \citep{wang2023cmb}{, }\\GeneTuring (Gene) \citep{jin2023genegpt}{, } EcomInstruct (Ecom) \citep{li2023ecomgpt}, leaf, text width=24em
                        ]
                    ]
                ]
                [
                    Analysis\\
                    (Sec \ref{sec:analysis})
                    [
                        Factuality Analysis\\
                        (Sec \ref{sec:factuality_analysis})
                        [
                            Knowledge Storage (Sec \ref{sec:analy_store})\\
                            Knowledge Completeness and Awareness (Sec \ref{sec:analy_aware})\\
                            Contextual Influence and Knowledge Conflict (Sec \ref{sec:analy_confict}), leaf, text width=27em 
                        ]
                    ]
                    [
                        Error Causes\\(Sec \ref{sec:causes})
                        [
                            Model-Level \ref{sec:model-causes}
                            [
                                Domain Knowledge Deficit{, } Outdated Information{, }\\ Immemorization{, } Forgetting{, } Reasoning Failure, leaf, text width=18em
                            ]
                        ]
                        [
                            Retrieval-Level \ref{sec:retrieval-causes}
                            [
                                Insufficient Information{, } Distracting Information{, } \\ Misinformation Not Recognized by LLMs{, }\\
                                Misinterpretation of Related Information, leaf, text width=18em
                            ]
                        ]
                        [
                            Inference-Level \ref{sec:inference-causes}
                            [
                                Snowballing{, } Erroneous Decoding{, } Exposure Bias, leaf, text width=18em
                            ]
                        ]
                    ]
                ]
                [
                    Enhancement\\ (Sec \ref{sec:enhancement})
                    [
                        On Standalone\\LLMs
                        (Sec \ref{sec:enhace_pure})
                        [
                            Pretrain-based
                            \ref{sec:enhace_pure}
                            [
                                Initial Pretraining: \citet{sadeq-etal-2023-unsupervised}{; }\\
                                Continual Pretraining: TOPICPREFIX \citep{lee2022factuality}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            SFT-based \ref{sec:enhace_pure_sft}
                            [
                                Continual SFT: \citet{moiseev-etal-2022-skill}{;}\\
                                Model Editing: \citet{dong-etal-2022-calibrating}{, }\\ CaliNET \citep{huang2023transformerpatcher}{, }  KN \citep{dai-etal-2022-knowledge}{, }\\ T-Patcher \citep{dai-etal-2022-knowledge}{, }
                                SERAC \citep{Mitchell2022MemoryBasedME}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Multi-Agent \ref{sec:enhace_pure_multi}
                            [
                                Multi-debate: \citet{multiagent_debate}\\
                                Multi-role: \citet{cohen2023lm}\\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Decoding \ref{sec:enhace_pure_decoding}
                            [
                                \citet{lee2022factuality}{,} \citet{chuang2023dola}\\
                                , leaf, text width=18em
                            ]
                        ]
                    ]
                    [
                        On Retrieval-\\Augmented\\LLMs(Sec \ref{sec:enhace_rag})
                        [
                            Normal RAG
                            \ref{sec:enhace_rag_normal})
                            [
                                \citet{borgeaud2022improving}{, } \citet{LlamaIndex} \\
                                , leaf, text width=18em
                            ]
                        ]
                        [
                            Interactive\\Retrieval \ref{sec:enhace_rag_inter}
                            [
                                CoT-based path: \citet{he2022rethinking}{, } IRCoT \citep{trivedi-etal-2023-interleaving} \\
                                Agent-based Retrieval: ReAct \citep{yao2023react}
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval\\Adaptation  \ref{sec:enhace_rag_adapt}
                            [
                                Prompt-based: LLM-Augmenter \citep{peng2023check}{, } \\
                                SFT-based: ATLAS \citep{Atlas}{, } \\REPLUG \citep{REPLUG}{, } SAIL \citep{luo2023sail}  \\
                                RLHF-based: GopherCite \citep{GopherCite}\\
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval on External \\ Memory \ref{sec:enhace_rag_mem}
                            [
                                 General Knowledge: \citet{li2022decoupled}{,}\\ \citet{houlsby2019parameterefficient}{,} G-MAP \citep{wan2022gmap}  \\
                                Entity Knowledge: knowledge plugin \citep{zhang-etal-2023-plug}\\KALA \citep{KALA} TOME \citep{jong2022mention}{, }  \\
                                , leaf, text width=16em
                            ]
                        ]
                        [
                            Retrieval on\\Structured Data
                            \ref{sec:enhace_rag_kg}
                            [
                                StructGPT \citep{StructGPT} {, } \citet{zhang2023mitigating}
                                , leaf, text width=16em
                            ]
                        ]
                    ]
                    [
                        Domain Factuality\\Enhanced LLMs
                        \\(Sec \ref{sec:domain_llms})
                        [
                            Medicine: HuatuoGPT \citep{zhang2023huatuogpt}{, } DISC-MedLLM \citep{ross2022large}\\
                            Legal: LawGPT \citep{nguyen2023brief}{, } ChatLaw \citep{cui2023chatlaw}\\
                            Finance: EcomGPT \citep{li2023ecomgpt}{, } BloombergGPT \citep{BloombergGPT} \\
                            Education: GrammarGPT \citep{fan2023grammargpt}\\
                                , leaf, text width=18em
                        ]
                    ]
                ]
            ]
        \end{forest}
    \end{adjustbox}
        \vspace{-4mm}
    \caption{Taxonomy of research on factuality in Large Language Models that consists of the issue, evaluation, analysis and enhancement.}
    \label{fig:tree}
\end{figure*}

==> tables/tb-enhancement-backup.tex <==

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t]
% \centering
% \caption{Performance of Factuality Enhancement Methods. We present the performance of baselines and the }
% \label{tab:enhance-table}
% \vspace{-4mm}
%   \setlength{\tabcolsep}{2.9mm}
%     \renewcommand{\arraystretch}{1.2}
% {\begin{tabular}{cccc}
% \toprule 
% Reference & Dataset & Metrics & Baselines $\rightarrow$ Theirs \\
% \midrule 
% \cite{li2022decoupled} & NQ~\citep{NQ} & EM & 34.5 $\rightarrow$ 44.35 (T5 11B) \\
% & GSM8K~\citep{cobbe2021training} & ACC & 77.0 $\rightarrow$ 85.0 (ChatGPT) \\
% \midrule 
% \cite{yu2023generate} & NQ~\citep{NQ} & EM & 20.9 $\rightarrow$ 28.0 (InstructGPT) \\
% % & TriviaQA~\citep{TQ} & EM & 57.5 $\rightarrow$ 59.0 (InstructGPT) \\
% & WebQA~\citep{WQ} & EM & 18.6 $\rightarrow$ 24.6 (InstructGPT) \\
% \midrule 
% \cite{chuang2023dola} & FACTOR News~\citep{muhlgay2023generating} & ACC & 58.3 $\rightarrow$ 62.0 (LLaMa-7B) \\
% % & & & 61.1 $\rightarrow$ 62.5 (LLaMa-13B) \\
% % & & & 63.8 $\rightarrow$ 65.4 (LLaMa-33B) \\
% & & & 63.6 $\rightarrow$ 66.2 (LLaMa-65B) \\
% % & FACTOR Wiki~\citep{muhlgay2023generating}  & ACC & 58.6 $\rightarrow$ 62.2 (LLaMa-7B) \\
% % & & & 62.6 $\rightarrow$ 66.2 (LLaMa-13B) \\
% % & & & 69.5 $\rightarrow$ 70.3 (LLaMa-33B) \\
% % & & & 72.2 $\rightarrow$ 72.4 (LLaMa-65B) \\
% & TruthfulQA~\citep{TruthfulQA} & \%Truth * Info & 32.4 $\rightarrow$ 44.6 (LLaMa-13B) \\
% & & & 34.8 $\rightarrow$ 49.2 (LLaMa-65B) \\
% \midrule 
% \cite{li2022contrastive} & TruthfulQA~\citep{TruthfulQA} & \%Truth * Info & 32.4 $\rightarrow$ 44.4 (LLaMa-13B) \\
% % & & & 31.7 $\rightarrow$ 36.7 (LLaMa-33B) \\
% & & & 34.8 $\rightarrow$ 43.4 (LLaMa-65B) \\
% \midrule 
% \cite{li2023inferencetime} & NQ~\citep{NQ} & ACC & 46.6 $\rightarrow$ 51.3 (LLaMA-7B) \\
% % & TriviaQA~\citep{TQ} & ACC & 89.6 $\rightarrow$ 91.1 (LLaMA-7B) \\
% & MMLU~\citep{hendrycks2020measuring}& ACC  & 35.7 $\rightarrow$ 40.1 (LLaMA-7B) \\
% & TruthfulQA~\citep{TruthfulQA} & \%Truth * Info & 32.5 $\rightarrow$ 65.1 (Alpaca) \\
% & & & 51.5 $\rightarrow$ 74.0 (Vicuna) \\
% & & & 26.9 $\rightarrow$ 43.5 (LLaMa-7B) \\
% \midrule
% \cite{cohen2023lm} & LAMA~\citep{LAMA} & F1 & 50.7 $\rightarrow$ 80.8 (ChatGPT) \\
%  % & TriviaQA~\citep{TQ} & F1 & 56.2 $\rightarrow$ 82.6 (ChatGPT) \\
%  & NQ~\citep{NQ} & F1 & 60.6 $\rightarrow$ 79.1 (ChatGPT) \\
%  & PopQA~\citep{PopQA} & F1 & 65.2 $\rightarrow$ 85.4 (ChatGPT) \\
%  % & LAMA & F1 & 42.5 $\rightarrow$ 79.3 (GPT-3) \\
%  % & TriviaQA~\citep{TQ} & F1 & 46.7 $\rightarrow$ 77.2 (GPT-3) \\
%  % & NQ~\citep{NQ} & F1 & 52.0 $\rightarrow$ 78.0 (GPT-3) \\
%  % & PopQA & F1 & 43.7 $\rightarrow$ 77.4 (GPT-3) \\
% \midrule
% \cite{weller2023according} & TriviaQA~\citep{TQ} & QUIP & 31.6 $\rightarrow$ 33.6 (ChatGPT) \\
%  % & NQ~\citep{NQ} & QUIP & 32.8 $\rightarrow$ 34.3 (ChatGPT) \\
%  % & HotpotQA~\citep{hotpotqa} & QUIP & 28.3 $\rightarrow$ 29.2 (ChatGPT) \\
%  & ELI5~\citep{ELI5}  & QUIP & 24.1 $\rightarrow$ 26.5 (ChatGPT) \\ 
%  % & TriviaQA~\citep{TQ} & EM & 77.8 $\rightarrow$ 78.8 (ChatGPT) \\
%  & NQ~\citep{NQ} & EM & 32.9 $\rightarrow$ 34.8 (ChatGPT) \\
%  & HotpotQA~\citep{hotpotqa} & F1 & 35.7 $\rightarrow$ 36.6 (ChatGPT) \\
%  & ELI5~\citep{ELI5}  & R-L & 22.7 $\rightarrow$ 21.7 (ChatGPT) \\
% \midrule
% \cite{dhuliawala2023chain} & MultiSpanQA~\citep{multispanqa} & F1 & 0.39 $\rightarrow$ 0.48 (LLaMA 65B) \\
%  & - & FactScore & 55.9 $\rightarrow$ 71.4 (LLaMA 65B) \\
%  & - & Avg. \# facts & 12.3 $\rightarrow$ 16.6 (LLaMA 65B) \\
% \midrule
% \cite{yao2023react} & HotpotQA~\citep{hotpotqa} & EM & 28.7 $\rightarrow$ 35.1 (PaLM-540B) \\
%  & FEVER~\cite{fever} & ACC & 57.1 $\rightarrow$ 62.0 (PaLM-540B) \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


==> tables/tb-eval-eval-benchmark.tex <==
\begin{table*}[]\small
\caption{Benchmarks for Evaluating the Factual Checker of LLMs}
\centering
\label{tab:eval_llms}
\vspace{-2mm}
  \setlength{\tabcolsep}{1.2mm}
{

\begin{tabular}{llllcll}
\toprule
Reference& \makecell[l]{Target\\Task} & Task & Dataset(Domain) & Metrics & \makecell[l]{Evaluated\\Checker}  \\
\midrule 
\citep{wang2023evaluating} &
Open QA &
QA-Eval &
EVOUNA &
\begin{tabular}[c]{@{}l@{}} 
ACC\\F1
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
Lexical Match,\\
BERTScore\\
GPT3.5
\end{tabular}
\\

\citep{FActScore} &
&
\begin{tabular}[c]{@{}l@{}} 
Factual Precision\\ of LLMs
\end{tabular}&
Biographies&
\begin{tabular}[c]{@{}l@{}} 
F1
\end{tabular}&
\begin{tabular}[c]{@{}l@{}} 
GPT-3.5\\
ChatGPT\\
Perplexity AI
\end{tabular}
\\

\citep{TRUE_re-evaluating}&
&
\begin{tabular}[c]{@{}l@{}} 
Factual\\Consistency\\ of NLG\end{tabular}&
\begin{tabular}[c]{@{}l@{}} 
FRANK,\\
SummEval,\\
MNBM,\\
QAGS-CNNDM,\\
QAGS-XSum,\\
BEGIN,\\
Q2,\\
DialFact,\\
FEVER,\\
VitaminC,\\
PAWS
\end{tabular}&
\begin{tabular}[c]{@{}l@{}} 
ROC-AUC\end{tabular}&
\begin{tabular}[c]{@{}l@{}} 
Q2,\\
ANLI,\\
SCzs,\\
F1,\\
BLEURT,\\
QuestEval,\\
FactCC,\\
BARTScore,\\
BERTScore
\end{tabular}
\\
\citep{nimah-etal-2023-nlg}&
&
\begin{tabular}[c]{@{}l@{}}
Controllable\\Generation
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
UBER-PPLM,\\
CTRL,\\
CTRL-Eval UBER,\\
USR Persona chat,\\
USR Topical chat,\\
SummEval,\\
Newsroom,\\
UniEval,\\ SummEval...
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
correlation,\\
human preference,\\
Kolmogorov-\\Smirnov
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
BLEU,\\
ROUGE,\\
BERTScore,\\
Perplexity,\\
CTC,\\
CTRLEval,\\
UniEval
\end{tabular}
\\

\bottomrule
\end{tabular}}
\end{table*}
